Study of multiple ring ELVES with the Mini-EUSO telescope on-board the International Space Station

Mini-EUSO (Multiwavelength Imaging New Instrument for the Extreme Universe Space Observatory) is a telescope observing the Earth in the ultraviolet band (290-430 nm) from the Russian Zvezda module of the International Space Station since 2019. The telescope is capable of observing UV emissions of cosmic, atmospheric, and terrestrial origin on different time scales. Among the atmospheric phenomena that can be studied, ELVES (Emission of Light and Very low-frequency perturbations due to Electromagnetic pulse Sources) have been photographed by Mini-EUSO with a time resolution of 2.5 us. ELVES are rapidly expanding rings of optical and ultraviolet emissions, 75-95 km in height, resulting from the de-excitation of molecular nitrogen and oxygen in the lower ionosphere following a lightning-associated ElectroMagnetic wave Pulse (EMP). A detailed study of their characteristics, such as radius, speed, and energy, is required for the understanding of these phenomena. In this work, results from the observation of about 30 ELVES with Mini-EUSO will be presented. Using dedicated algorithms, their electro-optical dynamics and morphological characteristics have been thoroughly investigated.

==> JEM-EUSO_Authors_July2023.tex <==
\newpage
\noindent
{\Large\bf Full Authors list: The JEM-EUSO Collaboration\\}
%{\scriptsize (author-list as of July 1st, 2023)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{fq}$, 
J.H.~Adams Jr.$^{pd}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{pd}$,
L.~Anchordoqui$^{pe}$,
A.~Anzalone$^{eh,ed}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{ph}$,
B.~Baret$^{cb}$,
D.~Barghini$^{el,ek}$,
M.~Battisti$^{ek,el,cb}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{kb}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{pf}$,
M.~Bianciotto$^{ek,el}$,
P.L.~Biermann$^{db}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{ft}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{na}$,
S.~Briz$^{pb}$,
J.~Burton$^{pd}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{de}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ft,ei, ej}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{bb}$,  
M.J.~Christl$^{pf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{en,ei}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{pa}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$, 
A.~de Castro G\'onzalez$^{pb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{pb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
A.~Ebersoldt$^{db}$,
T.~Ebisuzaki$^{ft}$,
J.~Eser$^{pb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{pc}$, 
W.W.~Finch$^{pc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{en,ei}$,
D.~Fuhne$^{pc}$,
C.~Fuglesang$^{na}$, 
M.~Fukushima$^{fe}$, 
S.~Gadamsetty$^{ph}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{kb}$, 
E.~Gazda$^{ph}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{pb}$,
A.~Haungs$^{db}$,
T.~Heibges$^{pc}$,,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{pa}$, 
F.~Kajino$^{ff}$, 
I.~Kaneko$^{ft}$, 
M.~Kleifges$^{db}$,
P.A.~Klimov$^{kb}$,
I.~Kreykenbohm$^{da}$, 
J.F.~Krizmanic$^{pj}$, 
V.~Kungel$^{pc}$,  
E.~Kuznetsov$^{pd}$, 
F.~L\'opez~Mart\'inez$^{pb}$, 
D.~Mand\'{a}t$^{bc}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ia}$, 
J.N.~Matthews$^{pg}$, 
A.~Menshikov$^{db}$,
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{pb}$,
J.~Mimouni$^{ad}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fi}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{ft}$, 
J.~M.~Nachtman$^{pi}$,
D.~Naumov$^{ka}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fe}$, 
T.~Ogawa$^{ft}$, 
S.~Ogio$^{ft}$, 
H.~Ohmori$^{ft}$, 
A.V.~Olinto$^{pb}$,
Y.~Onel$^{pi}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{ph}$,  
A.~Pagliaro$^{eh,ed}$,  
B.~Panico$^{ef, eg}$,  
E.~Parizot$^{cb, cd}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{pe}$,
M.~Pech$^{bc}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{ib}$,
Z.~Plebaniak$^{ei, ej}$, 
J.~Posligua$^{pi}$,
M.~Potts$^{ph}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ia}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{pd}$, 
M.H.~Reno$^{pi}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{ph}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fe}$, 
N.~Sakaki$^{ft}$, 
A.~Santangelo$^{dd}$, 
O.A.~Saprykin$^{kc}$,
F.~Sarazin$^{pc}$,
M.~Sato$^{fo}$, 
H.~Schieler$^{db}$,
P.~Schov\'{a}nek$^{bc}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$
S.A.~Sharakin$^{kb}$,
K.~Shinozaki$^{ia}$, 
S.~Stepanoff$^{ph}$,
J.F.~Soriano$^{pe}$,
J.~Szabelski$^{ia}$,
N.~Tajima$^{ft}$, 
T.~Tajima$^{ft, pn}$,
Y.~Takahashi$^{fo}$, 
M.~Takeda$^{fe}$, 
Y.~Takizawa$^{ft}$, 
C.~Tenzer$^{dd}$,
S.B.~Thomas$^{pg}$, 
L.G.~Tkachev$^{ka}$,
T.~Tomida$^{fh}$, 
S.~Toscano$^{ob}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,kb}$,
K.~Tsuno$^{ft}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.~M.~Venters$^{pj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ia}$, 
S.~Wada$^{ft}$,  
J.~Watts~Jr.$^{pd}$, 
A.~Weindl$^{db}$,
L.~Wiencke$^{pc}$, 
J.~Wilms$^{da}$,
D.~Winn$^{pm}$,
H.~Wistrand$^{pc}$,
I.V.~Yashin$^{kb}$, 
R.~Young$^{pf}$,
M.Yu.~Zotov$^{kb}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ad}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{bb}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bc}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cd}$ Institut universitaire de France (IUF)\\
% Germany - 4 institutes
$^{da}$ ECAP, University of Erlangen-Nuremberg, Germany\\
$^{db}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{dd}$ Institute for Astronomy and Astrophysics, Kepler Center, University of T\"ubingen, Germany\\
$^{de}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 15 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universita' degli Studi di Bari Aldo Moro and INFN - Sezione di Bari, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universita' di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universita' di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universita' di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universita' di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
% Japan - 7 institutes 
$^{fe}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{ff}$ Konan University, Kobe, Japan\\ 
$^{fh}$ Shinshu University, Nagano, Japan \\
$^{fi}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fo}$ Hokkaido University, Sapporo, Japan \\ 
$^{fq}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{ft}$ RIKEN, Wako, Japan\\
% Korea - 1 institute
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ia}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{ib}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ka}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{kb}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{kc}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{na}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ob}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 12 institutes 
$^{pa}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{pb}$ University of Chicago, IL, USA\\
$^{pc}$ Colorado School of Mines, Golden, CO, USA\\
$^{pd}$ University of Alabama in Huntsville, Huntsville, AL; USA\\
$^{pe}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{pf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{pg}$ University of Utah, Salt Lake City, UT, USA\\
$^{ph}$ Georgia Institute of Technology, USA\\
$^{pi}$ University of Iowa, Iowa City, IA, USA\\
$^{pj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{pm}$ Fairfield University, Fairfield, CT, USA\\
$^{pn}$ Department of Physics and Astronomy, University of California, Irvine \\
}

